Unified Text-Image Generation with Weakness-Targeted Post-Training

Unified multimodal generation architectures that jointly produce text and images have recently emerged as a promising direction for text-to-image (T2I) synthesis. In one approach, the model first generates a textual reasoning trace, and a manual modality switch in the inference pipeline then starts image generation. We study reward-weighted post-training with fully self-generated synthetic data for this reasoning-conditioned generation mode on BAGEL, a 14B mixture-of-transformers model that pairs autoregressive text generation with flow-matching image synthesis. Our post-training enables a learned modality switch, so the model itself can trigger image generation after its reasoning. We train on prompts that target the model's generation weaknesses, which yield better results than general image-caption or benchmark-derived prompts, a gain we do not attribute to weakness targeting alone. Our approach improves multimodal image generation on object-centric prompt alignment and text rendering, while remaining comparable on dense-prompt alignment and knowledge-intensive generation. We examine the impact of joint text-image generation on T2I performance and the relative importance of each modality during post-training. We apply the reward weight to the text loss, the image loss, or both, and compare against image-only post-training on the same images and reward labels. These modality ablations show that weighting both losses is most effective, and that reward weighting outperforms supervised fine-tuning in both multimodal and image-only post-training, especially for text rendering. A comparison of the two generation modes shows that reasoning helps on knowledge-intensive prompts, while image-only generation remains stronger on dense-prompt alignment and text rendering.

==> sec/single_sec_modality_experiments.tex <==
% Alt titles: 
% Does Joint Text-Image Generation Improve Text-to-Image Performance?
%  The Impact of Text Generation in Multimodal Post-Training
\section{The Impact of Text Generation in Multimodal Post-Training}\label{sec:modality_experiments}

In this set of experiments, we investigate a key question for unified multimodal generative models: \textit{how much does joint text-image generation contribute to T2I performance?} 
Intuitively, using a unified model with strong language capabilities to generate text that guides image generation should improve T2I performance. However, multimodal models generally underperform image-only generation models, even on benchmarks requiring implicit knowledge and reasoning~\cite{wiseworldknowledgeinformedsemantic, qwenimagetechnicalreport, oneigbenchomnidimensionalnuancedevaluation}.

We address this question through systematic modality ablations, comparing multimodal post-training against image-only post-training as well as reward-weighting each modality. 
Our base model, BAGEL, uses a Mixture-of-Transformers architecture~\cite{mixtureoftransformerssparsescalablearchitecture} which enables selective training or freezing of modality-specific parameters. By training only image-specific parameters versus training both modalities jointly, we isolate and measure the impact of text generation on T2I performance. 
We additionally compare modality importance in RWR by selectively reward-weighting different loss components: text loss only (Text RWR), image loss only (Image RWR), or both losses jointly (Multimodal RWR). In all RWR runs, parameters for both modalities are trained---only the loss weighting varies across configurations.
We train on our MMGW dataset discussed in Section \ref{sec:multimodal_gen_weaknesses_dataset}, with training hyperparameters in \TODO{Appendix ...}. 
All training configurations process the same number of samples for the same number of steps, though the image-only SFT setting trains exclusively on images and omits text traces. 

\input{tables/geneval_modality}
\input{tables/dpg_modality}


\subsection{Quantitative Results}\label{sec:modality_experiments_results}
We measure T2I performance across 4 benchmarks: GenEval~\cite{geneval}, an object-based prompt alignment benchmark; DPG-Bench~\cite{dpgbench}, which evaluates prompt alignment on dense prompts; WISE~\cite{wiseworldknowledgeinformedsemantic}, a benchmark requiring implicit understanding and world knowledge for successful generations; and OneIG-Bench~\cite{oneigbenchomnidimensionalnuancedevaluation}, a very difficult benchmark with fine-grained evaluation spanning prompt-image alignment, text rendering, reasoning-generated content, stylization, and diversity. 

As seen in Table \ref{tab:geneval_modality}, Multimodal RWR acheives the best overall performance on GenEval. Multimodal SFT and all other RWR settings slightly improve over BAGEL's Multimodal performance, but notably Image-Only SFT degrades performance. These results show that multimodal training yields stronger results than image-only training, and reward-weighting both modalities is most effective.

DPG-Bench results in Table \ref{tab:dpgbench_modality} show that BAGEL's Image-Only generation outperforms all multimodal generation methods. 
Multimodal RWR is the best multimodal method, demonstrating a clear improvement over the corresponding BAGEL Multimodal baseline and narrowing the performance gap to the Image-Only baseline while outperforming both SFT settings and prior multimodal models across several subcategories. This suggests that while Image-Only generation remains advantaged on DPG-Bench, reward-weighting both modalities can yield measurable gains.

\input{tables/wise_modality}
\input{tables/oneig_modality}

WISE results in Table \ref{tab:wise_modality} show Multimodal RWR achieving the best overall score of 0.72.
Gains are especially strong in the Chemistry, Physics, and Space categories, indicating that joint reward-weighting of both modalities enhances implicit understanding and factual grounding. Image RWR does not yield improvements over the BAGEL Multimodal baseline and Text RWR slightly degrades performance, indicating that relying solely on uni-modal rewards limits performance. 
Both Image-Only and Multimodal SFT underperform the BAGEL Multimodal baseline, indicating that synthetic data must be reward-weighted for useful training. 
These findings suggest that Multimodal RWR provides a balanced and effective signal for improving knowledge-intensive T2I generation.

On OneIG-Bench (Table \ref{tab:oneigbench_modality}), we see that Image-Only models, particularly SD3.5 Large, attain the highest scores in Alignment, Text Rendering, and Reasoning capabilities. Note that OneIG-Bench's Diversity scores only account for intra-prompt variance between images with no consideration of prompt alignment or image quality. 
Across multimodal methods, Multimodal RWR achieves the best Text Rendering score and competitive performance in Reasoning and Style evaluations. 
The Text category of OneIG-Bench shows particularly interesting trends, where the the performance of Image-Only models is generally an order of magnitude higher than Multimodal models; specifically for BAGEL, Multimodal generation results in a 10x performance degradation compared to Image-Only generation. 
Multimodal RWR greatly remedies this performance drop, achieving a Text score of 0.189 compared to BAGEL Multimodal's 0.020, but cannot fully close the gap to BAGEL Image-Only (0.244).
These results indicate that text rendering tasks are a specific area in which text-image generation worsens performance compared to image-only generation. 
% TODO: here we could reference the "When Multimodal Generation Harms Text-to-Image Performance" section IF NEEDED
Taken together, these results highlight that while multimodal reward-weighting strategies can close some gaps, the strongest T2I results on very challenging tasks like those in OneIG-Bench are still obtained by image-only models. This suggests there is still substantial room for improving text-image synergy in unified multimodal frameworks.

% Notably, reward-weighting both modalities (Multimodal RWR) yields moderate improvements over the baseline BAGEL Multimodal and SFT variants, while reward-weighting image or text alone does not confer consistent benefits. 
% for multimodal models remain lower than image-only models, further illustrating the efficiency of specialized image-only architectures on this axis.
